FIXED: Frustratingly Easy Domain Generalization with Mixup

Domain generalization (DG) aims to learn a generalizable model from multiple training domains such that it can perform well on unseen target domains. A popular strategy is to augment training data to benefit generalization through methods such as Mixup~\cite{zhang2018mixup}. While the vanilla Mixup can be directly applied, theoretical and empirical investigations uncover several shortcomings that limit its performance. Firstly, Mixup cannot effectively identify the domain and class information that can be used for learning invariant representations. Secondly, Mixup may introduce synthetic noisy data points via random interpolation, which lowers its discrimination capability. Based on the analysis, we propose a simple yet effective enhancement for Mixup-based DG, namely domain-invariant Feature mIXup (FIX). It learns domain-invariant representations for Mixup. To further enhance discrimination, we leverage existing techniques to enlarge margins among classes to further propose the domain-invariant Feature MIXup with Enhanced Discrimination (FIXED) approach. We present theoretical insights about guarantees on its effectiveness. Extensive experiments on seven public datasets across two modalities including image classification (Digits-DG, PACS, Office-Home) and time series (DSADS, PAMAP2, UCI-HAR, and USC-HAD) demonstrate that our approach significantly outperforms nine state-of-the-art related methods, beating the best performing baseline by 6.5\% on average in terms of test accuracy. Code is available at: https://github.com/jindongwang/transferlearning/tree/master/code/deep/fixed.

==> tab/tb-activity.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\caption{Results on Cross-person, cross-position, and cross-dataset human activity recognition. Please refer to the appendix for the full results on each domain.}
\label{tb-activity}
\resizebox{.43\textwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
Method   & X-Person      & X-Position    & X-Dataset     & AVG           \\ \midrule
ERM*      & 69.7          & 30.6          & 33.3          & 44.5         \\ 
DANN*~\cite{ganin2016domain}& \underline{71.6}          & 32.6          & \underline{41.2}          & \underline{48.5}          \\ 
CORAL*~\cite{sun2016deep}    & 66.6          & 25.4          & 39.3          & 43.8          \\ 
Mixup*~\cite{zhang2018mixup}    & 69.9          & \underline{36.0}          & 37.0          & 47.7         \\ 
GroupDRO*~\cite{sagawa2019distributionally} & 67.6          & 24.3          &  38.8         & 43.5         \\ 
RSC*~\cite{huang2020self}      & 69.6          & 33.3          & 41.0          & 48.0           \\ 

MIX-ALL*~\cite{wang2020heterogeneous}  & 68.5          & 34.5          & 32.4          & 45.2           \\ 
ANDMask*~\cite{parascandolo2020learning}  & 68.7          & 35.6          & 39.7          & 48.0          \\
GILE~\cite{qian2021latent}     & 70.0          & -             & -             & -           \\ 
Ours     & \textbf{76.6} & \textbf{38.4} & \textbf{50.0} & \textbf{55.0} \\ \bottomrule
\end{tabular}%
}

\end{table}

==> tab/tb-imageall.tex <==
\begin{table*}[t!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccccc}
\toprule
\multicolumn{1}{l}{} & Target & ERM & DANN & CORAL & ANDMask & GroupDRO & RSC & Mixup &MIX-ALL& Jigen*&MixStyle* & \method \\ \midrule
\multirow{5}{*}{\rotatebox{90}{Digits-DG}} &M&97.55&\underline{97.77}&97.62&96.85&97.48&\textbf{97.78}&97.50&96.23&96.50&96.50&97.67\\
&MM&55.52&55.62&57.68&56.00&53.47&56.27&57.95&59.28&\underline{61.40}&\textbf{63.50}&56.72\\
&SV&59.98&61.85&57.82&59.47&55.63&62.38&54.75&54.73&63.70&\textbf{64.70}&\underline{64.17}\\
&SY&89.25&89.37&\underline{90.12}&88.17&\textbf{92.15}&89.25&89.80&83.57&74.00&81.20&88.73\\
&AVG&75.58&76.15&75.81&75.12&74.68&76.42&75.00&73.45&73.90&\underline{76.50}&\textbf{76.82} \\ \midrule
\multicolumn{1}{l}{} & Target & ERM & DANN & CORAL & ANDMask & GroupDRO & RSC & Mixup & MIX-ALL&MixStyle*&SagNet* & \method \\ \midrule
\multirow{5}{*}{\rotatebox{90}{PACS(18)}} &A&77.00&78.71&77.78&76.22&76.03&79.74&79.10&80.66&\underline{84.10}&83.58&\textbf{84.23}\\
&C&74.53&75.30&77.05&73.81&76.07&76.11&73.46&73.85&\textbf{78.80}&\underline{77.66}&\textbf{78.80}\\
&P&95.51&94.01&92.63&91.56&91.20&95.57&94.49&93.83&\underline{96.10}&95.47&\textbf{96.37}\\
&S&77.86&77.83&\underline{80.55}&78.06&79.05&76.64&76.71&76.05&75.90&76.30&\textbf{83.54}\\
&AVG&81.22&81.46&82.00&79.91&80.59&82.01&80.94&81.1&\underline{83.70}&83.25&\textbf{85.74} \\ \midrule
\multicolumn{1}{l}{} & Target & ERM & DANN & CORAL & ANDMask & GroupDRO & RSC & Mixup & MIX-ALL&Jigen*&SagNet* & \method \\ \midrule
\multirow{5}{*}{\rotatebox{90}{Office(18)}} &A&58.63&57.73&58.76&56.74&57.60&58.96&55.79&56.08&53.04&\underline{60.20}&\textbf{61.06}\\
&C&47.95&44.42&48.75&45.86&48.77&\underline{49.16}&47.88&46.9&47.51&45.38&\textbf{50.08}\\
&P&72.22&71.95&72.34&70.67&71.53&\underline{72.54}&71.95&72.07&71.47&70.42&\textbf{73.39}\\
&R&73.03&72.50&73.63&73.19&73.17&\underline{74.16}&72.83&73.93&72.79&73.38&\textbf{74.45}\\
&AVG&62.96&61.65&63.37&61.61&62.77&\underline{63.70}&62.11&62.24&61.20&62.34&\textbf{64.75}\\ \bottomrule
\end{tabular}%
}
\caption{Classification accuracy on three image classification benchmarks. 
The \textbf{bold} and \underline{underline} items are the best and second-best results. 
On Digits-DG dataset, M, MM, SV and SY correspond to MNIST, MNIST-M, SVHN and SYN respectively. 
On PACS dataset, A, C, P and S correspond to art-painting, cartoon, photo and sketch respectively. 
On OfficeHome dataset, A, C, P and R correspond to Art, CliPart, Product and Real-World respectively. 
18 means the backbone is ResNet18.}
\label{tab:img}
\end{table*}


\begin{table}[ht!]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{ccc cccc c}
\toprule
\multicolumn{1}{c}{Dataset} & ERM  & GroupDRO & Mixup & CORAL & DA-CORAL&Fish & \method  \\
\midrule
VLCS&77.4&77.2&77.7&77.1&\underline{78.2}&77.8&\textbf{81.0}\\
OfficeHome&67.5&66.9&\underline{69.0}&68.6&68.9&68.6&\textbf{71.4} \\
TerraInc&47.2&47.0&\underline{48.9}&46.4&48.1&45.1&\textbf{56.9}\\
AVG&64.0&63.7&\underline{65.2}&64.2&\underline{65.2}&63.8&\textbf{69.8}\\ 
\bottomrule
\end{tabular}%
}
\caption{Average classification accuracy on three image classification benchmarks compared with the results from DomainBed. 
The \textbf{bold} and \underline{underline} items are the best and second-best results. Please refer to the appendix for detailed results on each domain.}
\label{tab:img50}
\end{table}

==> tab/tb-ohome-vlcs-terra.tex <==
\begin{table}[t!]
\centering
\caption{Results on PACS, Office-Home, VLCS, TerraInc, and DomainNet (ResNet-50). Detailed results on each domain of each dataset are presented in appendix.}
\label{tb-home-vlcs-terra}
\resizebox{.48\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
Method   & PACS          & Office-Home   & VLCS          & TerraInc      & DomainNet     & AVG           \\ \midrule 
ERM      & 85.5          & 66.5          & 77.5          & 46.1          & 40.9          & 63.3          \\
DANN~\cite{ganin2016domain}     & 83.6          & 65.9          & 78.6          & 46.7          & 38.3          & 62.6          \\
CORAL~\cite{sun2016deep}     & 86.2          & 68.7          & 78.8          & 47.6          & 41.5          & 64.6          \\
Mixup~\cite{zhang2018mixup}    & 84.6          & 68.1          & 77.4          & 47.9          & 39.2          & 63.4          \\
GroupDRO~\cite{sagawa2019distributionally} & 84.4          & 66.0          & 76.7          & 43.2          & 33.3          & 60.7          \\
RSC~\cite{huang2020self}      & 85.2          & 65.5          & 77.1          & 46.6          & 38.9          & 62.7          \\
SagNet~\cite{nam2021reducing}   & 86.3          & 68.1          & 77.8          & 48.6          & 40.3          & 64.2          \\
V-Rex~\cite{krueger2021out}    & 84.9          & 66.4          & 78.3          & 46.4          & 33.6          & 61.9          \\
DA-CORAL~\cite{dubey2021adaptive} & 84.5          & 68.9          & 78.2          & 48.1          & 43.9          & 64.7          \\
mDSDI~\cite{bui2021exploiting}    & 86.2          & 69.2          & 79.0          & 48.1          & 42.8          & 65.1          \\
SWAD~\cite{cha2021swad}     & \underline{88.1}    & \underline{70.6}    & \underline{79.1}    & \underline{50.0}    & \underline{46.5}    & \underline{66.9}    \\
Ours     & \textbf{89.7} & \textbf{71.4} & \textbf{81.0} & \textbf{56.9} & \textbf{47.6} & \textbf{69.3} \\ \bottomrule
\end{tabular}%
}

\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table}[t!]
% \centering
% \caption{Results on PACS, Office-Home, VLCS, and TerraInc datasets (ResNet-50) using results on DomainBed. The detailed results on each domain of each dataset are in appendix.}
% \label{tb-home-vlcs-terra}
% \resizebox{.48\textwidth}{!}{%
% \begin{tabular}{lccccc}
% \toprule
% Method   & PACS          & Office-Home   & VLCS          & TerraInc      & AVG           \\
% \midrule
% ERM      & 85.5          & 66.5          & 77.5          & 46.1          & 68.9          \\
% DANN~\cite{ganin2016domain}     & 83.6          & 65.9          & 78.6          & 46.7          & 68.7          \\
% CORAL~\cite{sun2016deep}    & 86.2          & 68.7          & 78.8          & 47.6          & 70.3          \\
% Mixup~\cite{zhang2018mixup}    & 84.6          & 68.1          & 77.4          & 47.9          & 69.5          \\
% RSC~\cite{huang2020self}      & 85.2          & 65.5          & 77.1          & 46.6          & 68.6          \\
% SagNet~\cite{nam2021reducing}   & 86.3          & 68.1          & 77.8          & 48.6          & 70.2          \\
% V-Rex~\cite{krueger2021out}    & 84.9          & 66.4          & 78.3          & 46.4          & 69.0          \\
% DA-CORAL~\cite{dubey2021adaptive} & 84.5          & 68.9          & 78.2          & 48.1          & 69.9          \\
% mDSDI~\cite{bui2021exploiting}    & 86.2          & 69.2          & 79.0          & 48.1          & 70.6          \\
% T3A~\cite{iwasawa2021test}     & 85.6          & 69.2          & \underline{80.0}    & 47.3          & 70.5          \\
% SWAD~\cite{cha2021swad}     & \underline{88.1}    & \underline{70.6}    & 79.1          & \underline{50.0}    & \underline{72.0}    \\
% Ours     & \textbf{89.7} & \textbf{71.4} & \textbf{81.0} & \textbf{56.9} & \textbf{74.7} \\ \bottomrule
% \end{tabular}%
% }

% \end{table}

==> tab/tb-pacs-ohome-digit.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t!]
\centering
\caption{Results on PACS, Office-Home, and Digits-DG dataset. Detailed results for each domain are in appendix.}
% \caption{Results on PACS, Office-Home, and Digits-DG dataset. Note that not all methods report results on all datasets, thus we select some methods and put them in a table for better formats. For more results, please refer to the appendix.}
\label{tb-pacs-ohome-digit}
\resizebox{.48\textwidth}{!}{%
\begin{tabular}{lr|lr|lr}
\toprule
\multicolumn{2}{c|}{PACS (ResNet-18)}             & \multicolumn{2}{c|}{Office-Home (ResNet-18)}        & \multicolumn{2}{c}{Digits-DG}              \\ 
\multicolumn{1}{l}{Method} &
  \multicolumn{1}{c|}{AVG} &
  \multicolumn{1}{l}{Method} &
  \multicolumn{1}{c|}{AVG} &
  \multicolumn{1}{l}{Method} &
  \multicolumn{1}{c}{AVG} \\ \midrule
ERM*        & 81.22          & ERM*            & 62.96          & ERM*            & 75.58          \\ 
DANN*~\cite{ganin2016domain} &

  81.46 &
  DANN*~\cite{ganin2016domain} &

  61.65 &
  DANN*~\cite{ganin2016domain} &

  76.15 \\ 
Mixup*~\cite{zhang2018mixup}      & 80.94          & CORAL*~\cite{sun2016deep}     & 63.37          & CORAL*~\cite{sun2016deep}      & 75.81          \\ 
InfoDrop~\cite{shi2020informative}  & 82.33          & Mixup*~\cite{zhang2018mixup}      & 62.11          & MMD-AAE~\cite{li2018domain1}   & 74.60           \\ 
GroupDRO*~\cite{sagawa2019distributionally}  & 80.59          & MMD-AAE~\cite{li2018domain1}    & 62.70           & Mixup*~\cite{zhang2018mixup}     & 75.00             \\ 
RSC*~\cite{huang2020self}       & 82.01          & Jigen~\cite{carlucci2019domain}      & 61.20           & Jigen~\cite{carlucci2019domain}      & 73.90           \\ 
ANDMask*~\cite{parascandolo2020learning}   & 79.91          & MIX-ALL*~\cite{wang2020heterogeneous}   & 62.24          & GroupDRO*~\cite{sagawa2019distributionally}    & 74.68          \\ 
MixStyle~\cite{zhou2021domain}   & 83.70           & GroupDRO*~\cite{sagawa2019distributionally}    & 62.77          & RSC*~\cite{huang2020self}         & 76.42          \\ 
SagNet~\cite{nam2021reducing}     & 83.25          & RSC*~\cite{huang2020self}       & \underline{63.70}           & MIX-ALL*~\cite{wang2020heterogeneous}  &  73.45          \\ 
StableNet~\cite{zhang2021deep} & \underline{84.69}          & ANDMask*~\cite{parascandolo2020learning}   & 61.61          & MixStyle~\cite{zhou2021domain}   & \underline{76.50}           \\ 
MatchDG~\cite{mahajan2021domain}   & 83.21          & SagNet~\cite{nam2021reducing}     & 62.34          & ANDMask*~\cite{parascandolo2020learning}   & 75.12          \\ 
Ours         & \textbf{85.74} & Ours          & \textbf{64.75} & Ours            & \textbf{76.82} \\ \bottomrule
\end{tabular}%
}

\end{table}
